Multimodal Prompt Retrieval for Generative Visual Question Answering

Recent years have witnessed impressive results of pre-trained vision-language models on knowledge-intensive tasks such as visual question answering (VQA). Despite the recent advances in VQA, existing methods mainly adopt a discriminative formulation that predicts answers within a pre-defined label set, leading to easy overfitting on low-resource domains with limited labeled data (e.g., medicine) and poor generalization under domain shift to another dataset. To tackle this limitation, we propose a novel generative model enhanced by multimodal prompt retrieval (MPR) that integrates retrieved prompts and multimodal features to generate answers in free text. Our generative model enables rapid zero-shot dataset adaptation to unseen data distributions and open-set answer labels across datasets. Our experiments on medical VQA tasks show that MPR outperforms its non-retrieval counterpart by up to 30% accuracy points in a few-shot domain adaptation setting.

==> tables/consistencies.tex <==
\begin{table}[t]    
    \footnotesize
    \renewrobustcmd{\bfseries}{\fontseries{b}\selectfont}

    \caption{Consistency of retrieval using our generative architecture. The GT column indicates what percentage of retrieved answers match ground truth. Similarly, prediction and question type columns indicate the proportion of retrieved answers that match model prediction and have correct question type respectively.}

    \centering
    \resizebox{\linewidth}{!}
    {
        \begin{tabular}{cSSSS}
        \hline
        \toprule[1pt]
       
         Train Data & Test Data & GT & Prediction & Question Type  \\

       
        % Method & {En$\rightarrow$FR} & {En$\rightarrow$KO}\\
        
        \hline

        SLAKE & SLAKE & 57.0 & 58.7 & 91.9  \\
        VQA-RAD & SLAKE & 57.0 & 39.9 & 91.9  \\
        VQA-RAD & VQA-RAD & 28.6 & 29.5 & 70.2  \\
        SLAKE & VQA-RAD & 28.6 & 31.8 & 70.2  \\
        
        % VecMap    & 28.4& 44.1 & 13.0 & 26.8 & 13.7&27.3\\
        \bottomrule[1pt]
        \end{tabular}
    }
    \label{tab:consistencies}

\end{table}

==> tables/further_finetune.tex <==
\begin{table}[t]    
    \footnotesize
    \renewrobustcmd{\bfseries}{\fontseries{b}\selectfont}

   

    \centering
    \resizebox{\linewidth}{!}
    {
        \begin{tabular}{cc|cc|cc}
        \hline
        \toprule[1pt]
       
         Train & Target & FT Train & RET Train & FT Target & RET Target  \\
    
       
        % Method & {En$\rightarrow$FR} & {En$\rightarrow$KO}\\
        
        \hline

        VQA-RAD & SLAKE &  59.5 & 67.8 & 66.2 & 51.3 \\
        % VQA-RAD & SLAKE &  67.8 & 51.3 \\

        SLAKE & VQA-RAD &  57.7 & 73.5 & 67.8 & 57.1 \\
        % SLAKE & VQA-RAD &  73.5 & 57.1  \\

        Both & Both & 76.7 & 71.1  & 76.7 & 71.1   \\
        % SLAKE + VQA-RAD & SLAKE + VQA-RAD &  71.1 & 71.1  \\
        
        % VecMap    & 28.4& 44.1 & 13.0 & 26.8 & 13.7&27.3\\
        \bottomrule[1pt]
        \end{tabular}
    }
     \caption{\tim{Maybe replace this with the graph in the appendix?}Continued finetuning across datasets. FT indicate that the model is trained on the train data, and then further finetuned on the target dataset. RET indicates that the model is not finetuned, instead using retrieval with k = 1 examples to evaluate on the target dataset. }
    \label{tab:further_finetune}

\end{table}

==> tables/question_categories.tex <==
\begin{table}[t]    
    \footnotesize
    \renewrobustcmd{\bfseries}{\fontseries{b}\selectfont}

    \caption{More specific question category performances with varying degrees of retrieval dataset access. The train dataset was SLAKE, and zero shot performance is evaluated on the VQA-RAD dataset. Horizontally adjacent gray cells indicate an improvement in accuracy when increasing retrieval set size. }

    \centering
    \resizebox{\linewidth}{!}
    {
        \begin{tabular}{cSSSS}
        \hline
        \toprule[1pt]
         Question Category & None & Train & Train + ROCO \\

       
        % Method & {En$\rightarrow$FR} & {En$\rightarrow$KO}\\
        \hline
        Abnormality & 50.0 & 33.9 & 33.9 \\
        Attribute & \cellcolor[gray]{0.8} 15.0 & \cellcolor[gray]{0.8} 50.0 & 50.0  \\
        Color  & \cellcolor[gray]{0.8} 0 & \cellcolor[gray]{0.8} 75.0 & 75.0  \\
        Modality  & 51.5 & \cellcolor[gray]{0.8} 39.4 & \cellcolor[gray]{0.8} 51.5  \\
        Organ & 40.0 & \cellcolor[gray]{0.8} 40.0 & \cellcolor[gray]{0.8} 50.0  \\
        Other & \cellcolor[gray]{0.8} 3.8 & \cellcolor[gray]{0.8} 15.4 & \cellcolor[gray]{0.8} 19.2  \\
        Plane & \cellcolor[gray]{0.8} 23.1 & \cellcolor[gray]{0.8} 69.2 & 65.4 \\
        Position  & \cellcolor[gray]{0.8} 8.2 & \cellcolor[gray]{0.8} 13.1 & 13.1  \\
        Presence  & \cellcolor[gray]{0.8} 43.3 & \cellcolor[gray]{0.8} 49.1 & 49.7 \\
        Quantity  & 33.3 & 16.7 & 16.7 \\
        Size  & \cellcolor[gray]{0.8} 41.3 & \cellcolor[gray]{0.8} 50.0 & 47.8 \\
        
        \bottomrule[1pt]
        \end{tabular}
    }
    \label{tab:question_categories}

\end{table}
